Fully Characterizing Lossy Catalytic Computation

A catalytic machine is a model of computation where a traditional space-bounded machine is augmented with an additional, significantly larger, "catalytic" tape, which, while being available as a work tape, has the caveat of being initialized with an arbitrary string, which must be preserved at the end of the computation. Despite this restriction, catalytic machines have been shown to have surprising additional power; a logspace machine with a polynomial length catalytic tape, known as catalytic logspace ($CL$), can compute problems which are believed to be impossible for $L$. A fundamental question of the model is whether the catalytic condition, of leaving the catalytic tape in its exact original configuration, is robust to minor deviations. This study was initialized by Gupta et al. (2024), who defined lossy catalytic logspace ($LCL[e]$) as a variant of $CL$ where we allow up to $e$ errors when resetting the catalytic tape. They showed that $LCL[e] = CL$ for any $e = O(1)$, which remains the frontier of our understanding. In this work we completely characterize lossy catalytic space ($LCSPACE[s,c,e]$) in terms of ordinary catalytic space ($CSPACE[s,c]$). We show that $$LCSPACE[s,c,e] = CSPACE[\Theta(s + e \log c), \Theta(c)]$$ In other words, allowing $e$ errors on a catalytic tape of length $c$ is equivalent, up to a constant stretch, to an equivalent errorless catalytic machine with an additional $e \log c$ bits of ordinary working memory. As a consequence, we show that for any $e$, $LCL[e] = CL$ implies $SPACE[e \log n] \subseteq ZPP$, thus giving a barrier to any improvement beyond $LCL[O(1)] = CL$. We also show equivalent results for non-deterministic and randomized catalytic space.

==> B3_old.tex <==
%\subsection{The Space Complexity of Encoding and Decoding BCH Codes}

%Having established appropriate lemmas on the space complexity of solving linear systems and other arithmetic, we can now move on to analysing the space complexity of encoding and decoding BCH codes.

%\quinten{introduce BCH codes}

%We present the BCH encoding algorithm.

%\quinten{add encoding equation, etc.}
%\begin{algorithm}
%\caption{$Encode_{BCH}$}
%\label{alg:encoding}
%\begin{algorithmic}[1]
    \State \textbf{initialization}: We assume that Algorithm \ref{alg:initialization} has been performed in advance.
    \State Compute and store the $r_i'$.
    \State Solve Equation \ref{eq:encoding}.
    \State Store the solution. \\
    \Return (with the added entries, we have a codeword now)
\end{algorithmic}
\end{algorithm}

We now argue that this is space efficient.

\quinten{include initialization costs}
\begin{lemma}
    \label{lemma:encoding}
    It is possible to encode word of length $2^{r_n} - \delta$ with an alphabet $F_n = GF(2^{r_n})$ and distance $\delta$ as a codeword of length $2^{r_n}$ with an additional space overhead of $O(e \log n) = (4e + 5) r_n \lceil \log p \rceil + O(\log^2 r_n)$. This implements the function $Encode_{BCH}$. \quinten{remove function name?}
\end{lemma}
\begin{proof}
    We look at the space complexity of every step of the encoding procedure. The cost of initialization is $3 r_n \lceil \log p \rceil + O(1)$ by Lemma \ref{lemma:initialization}.
    \begin{enumerate}
        \item Initialization costs $3r_n \lceil \log p \rceil + O(\log r_n)$ space by Lemma \ref{lemma:initialization}.
        \item For step 2, use Algorithm \ref{alg:compute_checks}. This means we store $2e r_n \lceil \log p \rceil$ values and use $4e r_n \lceil \log p \rceil + 5 r_n \lceil \log p \rceil + O(\log r_n)$ space. 
        \item For step 3, we use Lemma \ref{lemma:linsys} which uses $(4e + 5) r_n \lceil \log p \rceil + O(\log^2 r_n)$ space.
    \end{enumerate}
    Overall, this adds up to to a space cost $(4e + 5) r_n \lceil \log p \rceil + O(\log^2 r_n)$.
\end{proof}

That completes encoding. We now move to our analysis of decoding. We review the mathematics of the decoding.

Now we describe the decoding algorithm $Decode_{BCH}$:

\begin{algorithm}
\caption{$Decode_{BCH}$}
\label{alg:decode}
\begin{algorithmic}[1]
    \State \textbf{Initialization}: We assume that Algorithm \ref{alg:initialization} has been performed in advance.
    \State Compute the syndrome using Algorithm \ref{alg:compute_checks}
    \State Compute the determinant $\Delta$ of linear system \ref{eq:decode_linsys} with $j = \delta - 1$. Use the method described in the proof of Lemma \ref{lemma:linsys}.
    \While{$\Delta = 0$ and $j > 0$}
    \State $j \leftarrow j - 2$
    \State Compute the determinant $\Delta$ of linear system \ref{eq:decode_linsys} with parameter $j$.
    \EndWhile
    \If{$\Delta = 0$}
    \State Terminate the algorithm (no errors detected).
    \EndIf
    \State Use Lemma \ref{lemma:linsys} to solve linear system \ref{eq:decode_linsys} with parameter $j$. 
    \For{$i \leftarrow 0; i < j; i \leftarrow i + 1$}
        \State Find the $i$th root, $x_i^{-1}$ of the error locator polynomial according to some ordering.
        \State Compute the quantity $\alpha_{x_i}^{-1} = \left( \prod_{y \in M, y \neq x} (1 - yx^{-1}) \right)^{-1}$
        \State Evaluate the evaluator polynomials and compute the errors by multiplying $\omega(x^{-1})$ by $\alpha_{x_i}^{-1}$.
        \State Correct the corresponding error.
    \EndFor \\
    \Return (up to $e$ errors have now been corrected)
\end{algorithmic}
\end{algorithm}

\begin{lemma}
    \label{lemma:decoding}
    Algorithm~\ref{alg:decode} can be performed with space overhead $O(e \log n) = (6 + 4e) r_n \lceil \log p \rceil + O(\log^2 r_n)$ including the cost of the initialization using Algorithm \ref{alg:initialization}.
    \quinten{this cost was changed!}
\end{lemma}
\begin{proof}
    We review the cost of Algorithm~\ref{alg:decode} step-by-step. Steps that use a trivial amount of space are omitted.
    \begin{enumerate}
        \item Initialization costs $3r_n \lceil \log p \rceil + O(\log r_n)$ space by Lemma \ref{lemma:initialization}.
        \item By Lemma \ref{lemma:compute_checks}, the cost of Algorithm \ref{alg:compute_checks} is $5r_n \lceil \log p \rceil + 2 \lceil \log \delta \rceil + O(\log s_i)$ not counting the space needed to store the irreducible polynomial. 
        \item Storing and computing a determinant using the method in the proof of Lemma \ref{lemma:linsys} costs $2e r_n \lceil \log p \rceil + O(\log^2 r_n + \log e)$ space using access to an irreducible polynomial given in the initialization. The counter uses space $O(\log e)$.
        \stepcounter{enumi}
        \stepcounter{enumi}
        \item Reuse space from step 3.
        \stepcounter{enumi}
        \stepcounter{enumi}
        \item Solving the linear system by Lemma \ref{lemma:linsys} uses space $4e r_n \lceil \log p \rceil + 5r_n \lceil \log p \rceil + O(\log^2 r_n + \log e)$. We can reuse space used in step 3.
        \stepcounter{enumi}
        \item Evaluating a degree $2e$ polynomial can be done via Horner's method. This uses one sum register, one double sized multiplication output register and one counter register. The multiplication output register has twice the size since before taking the remainder, the full product as a polynomial has to be stored. Since the irreducible polynomial has been precomputed, and we can compute remainders in place, we can evaluate a polynomial in additional space $3r_i \lceil \log p \rceil + \lceil \log 2e \rceil + O(\log r_i)$. 
            Iterating over all possible solutions uses an additional $r_i \lceil \log p \rceil$ space. This procedure can recycle the space used in step 11. We use an additional register size $\lceil \log 2e \rceil$ to find the $i$th root. Counting the space used to store the irreducible polynomial means that this costs space $(4e + 5)r_n + O(\log^2 r_n + \log e)$.
        \item We add a (double-sized) multiplication output register for multiplication, a register to maintain the product, and another set of registers to iterate over all possible roots.  Iterating over all roots not equal to $x^{-1}$ allows us to then compute $\alpha_{x_i}$. We then take the multiplicative inverse using Lemma \ref{lemma:mult_inverse}. Overall, this uses space $(4e + 6) + O(\log r_n)$ by reusing registers.
        \item Reusing the space from steps 11 and 12 we can compute the value of the error by multiplying $\omega(x^{-1})$ by $\alpha_{x_i}^{-1}$.
    \end{enumerate}
    This covers all steps of Algorithm \ref{alg:decode} with significant space costs. We ignore $O(\log \delta)$ space terms here since these are all $O(\log n)$. This adds us to $(6 + 4e) r_n \lceil \log p \rceil + O(\log^2 r_n)$ space.
\end{proof}

% misc other stuff

\subsection{misc other stuff}


This completes the basic arithmetic operations over the finite field $GF(q^r)$.
\begin{lemma}
    \label{lemma:arithmetic}
    Given a sequence of finite fields $F_n = GF(p^{r_n})$ for a constant prime $p$, it is possible to perform addition, negation, multiplication and compute the multiplicative inverse in space $O(\log |F_n|)$.
\end{lemma}
\begin{proof}
    We use Lemma \ref{lemma:mult_inverse} for the multiplicative inverse. For addition, negation and multiplication we use Lemma \ref{lemma:well_endowed_polys} to perform these operations together with Lemmas \ref{lemma:irred_polys} to compute an irreducible polynomial (the same one, which is saved in memory) and Lemma \ref{lemma:remainder} to compute remainders.
\end{proof}
\quinten{not used...}



==> ecc.tex <==
\section{Error Correction Perspective}

\subsection{The Single Error Case}

While the simulation of  Theorem \ref{thm:main} made use of use of the reversibility of catalytic Turing machines, an alternative approach is viable using error correcting codes. It is possible to use an approach inspired by the Hamming code \cite{Hamming50} to correct a single bit error. Suppose the data $c$ is stored in binary and indexed by $i = i_k \dots i_0$ where $i_k, \dots, i_0$ are the binary digits of $i$ when expressed in binary, so
\begin{equation}
    i = \sum_{l = 0}^k i_l 2^l
\end{equation}
The Hamming code can then be seen to compute the parity bits 
\begin{equation}
    b_l = \sum_{i : i_l = 1} c_i \pmod 2
\end{equation}
where $c$ represents the data, or the catalytic tape in our case. Implicitly, we assume that the length of $c$ is no longer than $2^k$. Suppose we calculate thte values $b_l$ before and after the catalytic computation. We label the values before $b_l$ and the values after $b_l'$. If exactly one error is made during the computation, then the index of that error is precisely
\begin{equation}
    i' = \sum_{l = 0}^k |b_l' - b_l| 2^l
\end{equation}
since the quantity $|b_l' - b_l|$ can be thought of as testing whether or not the position of the error occurs at an index where $i_l = 1$.

Conversely, one can see how this method also allows us to encode data using errors as described in the simulation of $\errCSPACE[s, c, e]$ by a $\CSPACE[s + e \log c, c]$ machine. We use the bits $b_i$ to store data and observe that a single bit-flip has the power to change all bits $b_i$. Using the error position identification process in reverse one can change $b_i$ to be any values one likes. 

\subsection{Generalising to Multiple Errors}

A generalisation to multiple errors can be achieved using BCH codes. In this case we focus on systematic versions of BCH codes. In particular, we are interested in encoding and decoding the catalytic in logspace. With some analysis, the method described in \cite{DodisReyzinSmith04,DodisOstrovskyReyzinSmith06} achieves this. The method they use avoids significant computational costs by avoiding the need to compute discrete logarithms. 



==> thm-for-old.tex <==
{\color{red} ECC ARGUMENT HERE}

\quinten{better outline of section --- one paragraph saying we use err corr codes}

\quinten{swap firstly secondly}
It is possible to use error correcting codes to correct errors in the catalytic tape. A rough sketch of how to use an error correcting code for simulating $M_e$ in three steps is as follows: First use an error correcting code to encode the catalytic tape using additional $O(e \log c)$ space for redundancy. Second, run the machine $M_e$ using the catalytic tape $c$ and clean space $s$ allowing it to make up to $e$ errors on the catalytic tape. Third, use the error correcting code to detect and correct the $e$ errors restoring the catalytic tape to original instatiation.
This procedure requires an error correcting code that can detect and correct up to $e$ errors.
Furthermore, for encoding a data string of length $|c|$ it can use at most $O(e \log c)$ additional redundant space to encode the codewords. Lastly, the operations required to encode and decode the catalytic tape must be accessible by a machine using at most $O(s + e \log c)$ space\footnote{Technically the machine could make use of the catalytic tape to do encoding and decoding, as long as it is a catalytic process, but the requirement of using at most $O(s + e \log c)$ is sufficient.}. We will show that BCH codes~\cite{original ref} adhere to all these three restrictions.

%In our case, we use BCH codes. We use BCH codes since they generalise the Hamming code. The Hamming code is an easy special case for correcting single errors.

%The first feature can be achieved by closely analysing the space complexity of the encoding and decoding procedures of certain codes. The second feature can be achieved for systematic codes with some extra work.

We use the description of BCH codes given by \cite{dodisreyzinsmith04,dodisostrovskyreyzinsmith06}. The main parameters of these codes can be summarised as followed.

\begin{itemize}
\item alphabet: $GF(q)$ for a prime $q$
\item length of words: $n = q^m - 1$ (this can be more general). For a catalytic tape of length $c$, $n = c = q^m - 1$.
\item distance: a parameter $\delta$. This affects the number of valid codewords.
\end{itemize}

BCH codes can be generalised beyond what is described above, but this suffices for our purposes. We will take $q = 3$ \marten{why 3 not 2?} in our procedure. We summarise the main components of our procedure to use BCH codes to correct errors on a catalytic tape.

\begin{enumerate}
    \item \textbf{Indexing}: BCH codes associate a particular value of the field $GF(q^m)$ (an index) with every position of a word. We compute these in a space efficient manner by iterated multiplication. 
    \item \textbf{Encoding}: The version of BCH codes we use are systematic which simplifies the process. But in order to turn the catalytic tape into a codeword, extra correction bits have to be computed. In particular, we use the extra $O(e \log c)$ clean space to extend the catalytic tape. The catalytic tape together with these extra bits together form a codeword. Finding these bits requires solving a linear system which can be done.
    \item \textbf{Decoding}: In order to decode the system we can use Berlekamp's decoding algorithm \cite{Berlekamp71} as described by \cite{dodisreyzinsmith04,dodisostrovskyreyzinsmith06}. The main computational steps are evaluating polynomials, solving a linear system and solving a polynomial. Since all of these steps occur over the finite field $GF(q)$ or $GF(q^m)$, this can be done efficiently.
\end{enumerate}

We present some helpful lemmas and definitions.



We now describe the components of the error correction procedure in more detail.

\paragraph{Indexing}
In a BCH code, position of a word is assigned an `index' $x \in \mathcal{F}^*$ where $\mathcal{F}^* = \mathcal{F} \setminus \{0\}$ for $\mathcal{F} = GF(q^{r_n})$. For both encoding and decoding it is necessary to compute $x$. It is known that the multiplicative group $\mathcal{F}^*$ associated with a finite field $\mathcal{F}$ is always cyclic. Therefore, if we pick any non-identity element $\alpha$ from $\mathcal{F}^*$ we have a generator. Since the catalytic tape is linear, we can associate any position $i$ on the tape with the index $x = \alpha^i$. Therefore, computing the index $x$ means computing the power function. 
Using the reasoning from the proof of Lemma \ref{lemma:linsys_l2} multiplication over $\mathcal{F}_q[\xi]$ can be in $\mathsf{NC}^1$ where the parameter is the length function so $O(d \log q)$ where $d$ is the degree of the polynomial. By Theorem 4 from \cite{Borodin77}, this means multiplication can be performed in space $O(\log d + \log \log q)$. 
We would like to use the algorithm described in the proof of Lemma~\ref{lemma:linsys_l2} to compute the corresponding value in $GF(q^m)$. However, this assumes access to an irreducible polynomials in order to make arithmetic over the field $GF(q^m)$ possible. In other words, it requires an irreducible polynomial of degree $m$ over the field $\mathbb{F}_q$. Such a polynomial requires space $O(m \log q) = O(\log c) = O(\log n)$ bits to store. By assumption, the catalytic machine has access to this amount of space. In order to find an irreducible polynomial, we iterate over all possible polynomials. It is known that such a polynomial must always exist, so we must eventually find one. In order to test whether or not a polynomial is irreducible or not, observe that since we have enough space to iterate over all possible polynomials up to degree $m$ we also have enough space to iterate over all possible pairs of polynomials up to degree $m$. The algorithm described in the proof of Lemma~\ref{lemma:linsys_l2} still works for computing remainders in space $O(\log m + \log \log q) = O(\log \log c) = O(\log \log n)$. Therefore, we can iterate over all candidate irreducible polynomials and all non-trivial factors to test whether or not the candidate is irreducible. Eventually, we find and store an irreducible polynomial in space $O(\log n)$ using this method.
Thus, using the algorithm described in the proof of Lemma \ref{lemma:linsys_l2} and the irreducible polynomial found above
\quinten{split lemma into parts?}
we can then compute the remainder in space $O(\log d + \log \log q)$. Since $|\mathcal{F}^*| = q^m - 1$ the degree $d \leq 2m$ and since $\mathcal{F}^*$ indexes the catalytic tape $|\mathcal{F}^*| = O(c)$ so one can compute the remainder in space $O(\log \log c)$.

Therefore multiplication over the field $GF(q^m)$ can be done in space $O(\log \log c)$. But multiplication may have to be repeated $O(c)$ times and therefore a clock size $O(\log c) = O(\log n)$ is necessary. Thus space $O(\log n + \log \log n) = O(\log n)$ is necessary to compute the index $x$. The catalytic machine has access to this amount of space. Finally, observe that repeated squaring is faster in time, but may require more space ($O(\log n \log \log n)$ naively). \quinten{repeated squaring fine?}

\paragraph{Encoding}
Codewords are defined to be the words that satisfy for all $i = 1, \dots, \delta - 1$
\begin{equation}
    r_i = \sum_{x \in \mathcal{F}^*} d_x x^i = 0
\end{equation}
where $d_x$ denotes the value of the cell indexed by $x$ on the catalytic tape. Using the indexing procedure above, $x$ can be computed space-efficiently. By earlier reasoning, multiplication with $d_x$ can also be done efficiently. By reasoning from the proof in Lemma \ref{lemma:linsys_l2}, the polynomial ring $\mathbb{F}_q[\xi]$ is well-endowed. As such, addition can be done in constant depth certainly space $O(\log \log c) = O(\log \log n)$ (the space if it were in $\mathsf{NC}^1$). But in order to iterate over all values of $\mathcal{F}^*$ we also use a clock size $O(\log c) = O(\log n)$. Therefore, we can compute the $r_i$ in space $O(\log n)$.

For an arbitrary catalytic tape, the $r_i$ need not be zero, but in order to correct errors later, we must start the computation on a codeword. We can make any catalytic tape into a codeword using the following trick. First, we count $(\delta - 1) \log c = O(\delta \log n)$ bits from the clean tape to catalytic tape. Since we will later set $\delta = O(e)$, we have access to this amount of clean space. Since these are clean tape bits, we can write anything we want on to them, but after initialisation we will count them as part of the catalytic tape for all intents and purposes. The purpose of these bits is to fill them with values such that taken as a whole, the new catalytic tape now corresponds exactly to a codeword. In particular, we will find that this works no matter the initial configuration of the original catalytic tape. Let $C \subseteq \mathbb{F}^*$ refer to subset of $\mathcal{F}^*$ that corresponds to the first $\delta - 1$ indices of the catalytic tape that actually resides on the clean tape. Now define the new quantities

\begin{equation}
    r_i' = \sum_{x \in \mathcal{F}^* \setminus C} d_x x^i = 0 \,.
\end{equation}

Now we observe that setting $r_i' = 0$ gives a linear system in the remaining $d_x$ for $x \in C$ with $\delta - 1$ unknowns and $\delta - 1$ equations. Furthermore, observe that this linear system written as a matrix equation uses a finite field Vandermonde matrix. Vandermonde matrices have explicit inverses (even in this finite field case) meaning that a solution always exists. Therefore, using Lemma~\ref{lemma:linsys_l2} we can solve this linear system efficiently, obtaining the solution as a numerator denominator pair. Also, observe from the earlier discussion in indexing \quinten{move to lemma} that we can compute the irreducible polynomial the lemma requires. We would like to have access to solution of the linear system, but not in numerator denominator form, so we would like to perform division. 
We can compute the inverse of an element in $GF(q^m)$ by iterating over all elements of $GF(q^m)$ and checking if their product equals 1 after computing the remainder. Using a clock and the space complexity of multiplication and remainder this costs $O(\log n + \log \log n)$ space and so is doable. Once we have found the inverse of the denominator, we can multiply it with the numerator to compute the solution to the linear system. \quinten{split into more lemmas...} Having found these values, we store and thus together with the original catalytic tape, the `new' catalytic tape is guaranteed to form a codeword. This completes the encoding step.

\paragraph{Decoding} Decoding follows the procedure described in \cite{dodisreyzinsmith04,dodisostrovskyreyzinsmith06} with some simplifications since we prioritise space over time. First, the syndrome $\mathsf{syn}(p)$ of a message $p$ is computed. The syndrome is defined as the collection of the $r_i$ values defined before. From the syndrome we compute the support of the error, $\mathsf{supp}(p) = \{(x, p_x)_{x : p_x \neq 9}\}$ which is defined as the value of the error $p_x$ together with its position $x$. Then the error can be `subtracted' from the word to give back the original codeword. The error correction method only works if the number of errors is less than $(\delta - 1)/2$ and hence we set $\delta = 2e + 3$ ($\delta$ being odd helps later). It is important for space efficiency that we store only the support of the error instead of a full error string which would require too much space. 
The support on the other hand uses exactly $O(e \log c)$ space.

The decoding algorithm is a variation of Berlekamp's BCH decoding algorithm. First define the following polynomials using $M = \{x \in \mathcal{F}^* | p_x \neq 0\}$
\begin{align}
\sigma(z) &= \sum_{x \in M} (1 - xz)
          &
\omega(z) &= \sigma \sum_{x \in M} \frac{p_x xz}{1 - xz}
\end{align}
\marten{should the sum in the definition of $\sigma(z)$ be a product? because now the degree of this polynomial will always be one?}
which both have degree at most $|M| \leq (\delta - 1)/2$. Here $\sigma(z)$ is known as the error locator polynomial since the multiplicative inverses of its roots are the locations of the errors. Similarly, $\omega(z)$ is known as the evaluator polynomial since it gives the error since $\omega(x^{-1}) = p_x \prod_{y \in M, y \neq x} (1 - yx^{-1})$. Note that since these polynomials have no common zeroes, $\mathrm{gcd}(\sigma(z), \omega(z)) = 1$. 

It turns out that $\sigma(z)$ and $\omega(z)$ are the almost unique solutions to the congruence
\begin{equation}
    S(z) \sigma(z) \equiv
    \omega(z) \pmod {z^\delta}
\end{equation}
where $S(z) = \sum_{l=1}^{\delta - 1} r_l z^l$. Suppose that $\sigma'(z),\omega'(z)$ are other solutions to this congruence then
\begin{equation}
    \omega(z) \sigma'(z) \equiv
    \sigma(z) S(z) \sigma'(z) \equiv
    \sigma(z) \omega'(z) \pmod {z^\delta} \,.
\end{equation}
Therefore if we restrict the degree of both $\omega(z)$ and $\sigma(z)$ to be polynomials of degree at most $(\delta - 1) / 2$ then as polynomials it is also true that $\omega(z) \sigma'(z) = \sigma(z) \omega'(z)$ and therefore that $\omega(z) / \sigma(z) = \omega'(z) / \sigma'(z)$. So if we also require that $\omega(z)$ and $\sigma(z)$ are relatively prime and $\sigma(z)$ has constant coefficient 1, then $\omega(z), \sigma(z)$ are unique.

After setting the constant term of $\sigma(z)$ to be 1, the above congruence gives a linear system with $\delta$ unknowns and $\delta$ equations with coefficients in the field $GF(q^m)$. We use almost the same procedure as described in the encoding step and making use of Lemma \ref{lemma:linsys_l2} in order to solve this system. If less than $(\delta - 1) / 2$ errors are made, a solution is guaranteed to exist. However, we cannot force $\sigma(z)$ and $\omega(z)$ to be coprime in the linear system and as a result the solution may not be unique. Suppose $\sigma(z)$ and $\omega(z)$ have a common factor $\tau(z)$. Since $\omega(z)$ must have a constant coefficient 1, the constant coefficient of $\tau(z)$ must also be 1. But then $\tau(z)$ must have degree at least 1 and therefore $\sigma(z)$ and $\omega(z)$ both have degree at least 1 too high.
Therefore, if more than one solution to the system exists, some of these solutions will have too high a degree. But we can test whether or not the system has more than one solution by evaluating the determinant of the matrix of that system. Using the approach described in Lemma \ref{lemma:linsys_l2}, we can evaluate this determinant. If this determinant is nonzero, we know a unique solution exists and so we can use the method from Lemma \ref{lemma:linsys_l2} to solve the system.
If the determinant is 0, we can repeat our procedure but now with $\delta$ replaced by $\delta - 2$ to get a smaller linear system. Repeating this procedure, either we find that the determinant is always 0, meaning that there are no errors to correct, or eventually that the determinant is nonzero and we can solve for polynomials $\sigma(z), \omega(z)$. For identical reasons to the encoding step, this can be done space efficiently.

\quinten{BCH excerpt makes some comments about distinct roots I do not understand}

Having solved for polynomials $\sigma(z)$ and $\omega(z)$ we can iterate over all possible values of $z \in \mathcal{F}^*$ to find all roots to $\sigma(z)$ and then compute their inverses using a similar procedure to that described in the encoding step. The evaluation of this polynomial can be done space efficiently, similar to the evaluation of $r_i$ but much simpler in fact. Afterwards, we can evaluate $\omega(z)$ to compute the errors. This is not necessary when $q = 2$ and the error is guaranteed to be 1. Once these have been computed, storing the support of the error is space efficient and the catalytic tape can be corrected. This completes the decoding step.

There are many types of BCH codes. The single error case, the Hamming code, can be described quite simply and is included in the appendix. Reed-Solomon codes are also BCH codes. They are more challenging to use in catalytic computation since they require one to use a changing alphabet size $q$ for a prime number $q$. Since the catalytic tape is written on a tape with a fixed alphabet, using $q = 2$ and then powers of $q$ for the BCH code is easier to implement for catalytic computation.

\quinten{Lemma \ref{lemma:linsys_l2} has weird grammar.}
\quinten{not working on the same field for decoding?}

\quinten{solve linear systems brute force? --- only helps slightly}
\marten{I think it would be good sumarize the above into one theorem that clearly states how the simulation is done. Something like below:}
